Functional Meaning for Parallel Streaming

Nondeterminism introduced by race conditions and message reorderings makes parallel and distributed programming hard. Nevertheless, promising approaches such as LVars and CRDTs address this problem by introducing a partial order structure on shared state that describes how the state evolves over time. Monotone programs that respect the order are deterministic. Datalog-inspired languages incorporate this idea of monotonicity in a first-class way but they are not general-purpose. We would like parallel and distributed languages to be as natural to use as any functional language, without sacrificing expressivity, and with a formal basis of study as appealing as the lambda calculus. This paper presents $\lambda_\vee$, a core language for deterministic parallelism that embodies the ideas above. In $\lambda_\vee$, values may increase over time according to a streaming order and all computations are monotone with respect to that order. The streaming order coincides with the approximation order found in Scott semantics and so unifies the foundations of functional programming with the foundations of deterministic distributed computation. The resulting lambda calculus has a computationally adequate model rooted in domain theory. It integrates the compositionality and power of abstraction characteristic of functional programming with the declarative nature of Datalog. This version of the paper includes extended exposition and appendices with proofs.

==> pp/figures/denot.tex <==
\begin{figure}[h]
\[
\begin{array}{lcl}
  \multicolumn{3}{l}{\disosym : \domval \cong (\ideals{\symset} + \domval \times \domval +
    \powdomh{\domval} + (\domval \to \domcomp))_\botv }\\
  \\
  \multicolumn{3}{l}{\monlift{(\mathemdash)} \in (\domval \to \domcomp) \to (\domcomp \to \domcomp)}\\
  \monlift{f}(d) &=&
  \begin{cases}
    \bot &\text{if } d = \bot\\
    \top &\text{if } d = \top\\
    f(d) &\text{if } d \in \domval
  \end{cases}
  \\

  \multicolumn{3}{l}{\monadpair{\mathemdash}{\mathemdash} \in \domcomp \times \domcomp \to \domcomp}\\
  \monadpair{d_1}{d_2} &=& \mathbind{d'_1}{d_1}{
    \mathbind{d'_2}{d_2}{\dfold{(d'_1, d'_2)}}} \\
  \\
  \multicolumn{3}{l}{\monadset{ \mathemdash } \in \powerset{\domcomp} \to \domcomp}\\
  \monadset{ d \in X } &=&
    \dfold{\bigcup_{d \in X}{(\mathbind{d'}{d}{\downclosk{d'}})}} \\
  \\
    \multicolumn{3}{l}{\denot{\mathemdash}{\mathemdash} \in \syncomp \times (\varset \to \domval) \to \domcomp} \\
    \denot{\mathit{x}}{\semsubstmeta} &= &\semsubstmeta(\mathit{x}) \\
    \denot{ \tmBotC }{\semsubstmeta} &= &\bot \\
    \denot{ \tmTopC }{\semsubstmeta} &= &\top \\
    \denot{ \valBotV }{\semsubstmeta} &= &\botv \\
    \denot{ \valLam{ \mathit{x} }{ \tmMeta } }{\semsubstmeta} &=
      & \dfold{\denot{e}{\extmap{\semsubstmeta}{\mathit{x}}{\mathemdash}}} \\
    \denot{ \tmPair{ \tmMeta }{ \tmMeta' } }{\semsubstmeta} &= & \monadpair{\denot{\tmMeta}{\semsubstmeta}}{\denot{\tmMeta'}{\semsubstmeta}} \\
    \denot{\ottnt{s}}{\semsubstmeta} &= & \dfold{\prinideal{\ottnt{s}}\,} \\
    \denot{\ottsym{\{}  \tmMeta_{{\mathrm{1}}}  \ottsym{,} \, ... \, \ottsym{,}  \tmMeta_{\ottmv{n}}  \ottsym{\}}}{\semsubstmeta} &=
    & \monadset{\denot{\tmMeta_{{\mathrm{1}}}}{\semsubstmeta}, \ldots, \denot{\tmMeta_{\ottmv{n}}}{\semsubstmeta}} \\
    \denot{ \tmApp{ \tmMeta_{{\mathrm{1}}} }{ \tmMeta_{{\mathrm{2}}} } }{\semsubstmeta} &=
      & \mathbind{d_1}{\denot{\tmMeta_{{\mathrm{1}}}}{\semsubstmeta}}
          {\begin{cases}
            \monlift{\dunfold{d_1}}(\denot{\tmMeta_{{\mathrm{2}}}}{\semsubstmeta})
              & \text{if } \dunfold{d_1} \in \contfun{\domval}{\domcomp} \\
                       \bot & \text{otherwise}
                     \end{cases}} \\
    \denot{\ottkw{let} \, \ottsym{(}  \mathit{x}  \ottsym{,}  \mathit{x'}  \ottsym{)}  \ottsym{=}  \tmMeta_{{\mathrm{1}}} \, \ottkw{in} \, \tmMeta_{{\mathrm{2}}}}{\semsubstmeta} &=
      & \mathbind{d_1}{\denot{\tmMeta_{{\mathrm{1}}}}{\semsubstmeta}}
          {\begin{cases}
              \denot{\tmMeta_{{\mathrm{2}}}}{\extmap{\extmap{\semsubstmeta}{\mathit{x}}{d}}{\mathit{x'}}{d'}} & \text{if } \dunfold{d_1} = (d, d') \\
             \bot & \text{otherwise}
           \end{cases}} \\
    \denot{\ottkw{let} \, \ottnt{s}  \ottsym{=}  \tmMeta_{{\mathrm{1}}} \, \ottkw{in} \, \tmMeta_{{\mathrm{2}}}}{\semsubstmeta} &=
      & \mathbind{d_1}{\denot{\tmMeta_{{\mathrm{1}}}}{\semsubstmeta}}
          {\begin{cases}
              \denot{\tmMeta_{{\mathrm{2}}}}{\semsubstmeta} & \text{if } \dunfold{d_1} \in \ideals{\symset} \text{ and } \ottnt{s} \in \dunfold{d_1}  \\
             \bot & \text{otherwise}
           \end{cases}} \\
    \denot{ \tmBigJoin{ \mathit{x} }{ \tmMeta }{ \tmMeta' } }{\semsubstmeta} &=
      & \mathbind{d}{\denot{\tmMeta}{\semsubstmeta}}
          {\begin{cases}
              \bigsemjoin{d' \in \dunfold{d}}{\denot{\tmMeta'}{\extmap{\semsubstmeta}{\mathit{x}}{d'}}} & \text{if } \dunfold{d} \in \powdomh{\domval} \\
             \bot & \text{otherwise}
           \end{cases}}\\
    \denot{ \tmJoin{ \tmMeta_{{\mathrm{1}}} }{ \tmMeta_{{\mathrm{2}}} } }{\semsubstmeta} &= & \semjoin{\denot{\tmMeta_{{\mathrm{1}}}}{\semsubstmeta}}
         {\denot{\tmMeta_{{\mathrm{2}}}}{\semsubstmeta}} \\
  \end{array}
\]
\caption{Scott-style \gcalc Denotational Semantics}
\label{fig:denot}
\end{figure}


==> pp/figures/eq.tex <==
\begin{figure}
  \drules[]{$ \ctxeq{ \tmMeta_{{\mathrm{1}}} }{ \tmMeta_{{\mathrm{2}}} } $}{equivalence}
         {eqtJoinAssoc, eqtJoinComm, eqtJoinIdemp, eqtBotIdent, eqtBotVIdent, eqtTopAbsorb,
          eqtLamBeta, eqtSymBeta, eqtPairBeta, eqtSetBeta,
          eqtLamEta, eqtSymEta, eqtPairEta, eqtSetEta,
          eqtVarCong, eqtLamCong, eqtPairCong, eqtSymCong,
          eqtSetCong, eqtAppCong, eqtLetPairCong,
          eqtLetSymCong, eqtSetJoinCong, eqtJoinCong
         }
  \todo{this figure is missing the ``stuck term'' cases}
  \caption{\gcalc Equational Theory}
  \label{fig:eq}
\end{figure}
\todo{}


==> pp/figures/reachability.tex <==
\begin{figure}[t]
  {
    \scriptsize

    \todo{diagram of a graph}

    \vspace{1em}

    \centering
    \begin{subfigure}[c]{0.32\textwidth}
      \begin{lstlisting}[language=Haskell]
reaches x = do
  x <- newEmptySet
  -- TODO
      \end{lstlisting}

      \caption{LVars}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.32\textwidth}
      \begin{lstlisting}[language=Prolog]
reaches(X, X).
reaches(X, Z) :-
  neighbors(X, Y),
  reaches(Y, Z).
      \end{lstlisting}

      \caption{Datalog}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.32\textwidth}
      \begin{lstlisting}[language=Haskell]
reaches x = {x} ∨
  (for n in neighbors x
   join (reaches n))
      \end{lstlisting}

      {
      \footnotesize
      \nr{Above: `for' should be bold. Not sure how to get good code formatting for Granite code. Also not sure how to fix the missing characters in the font.}
      }
    \caption{\gcalc}
    \label{fig:reachability:gcalc}
  \end{subfigure}
  }

  \caption{Graph reachability}
  \label{fig:reachability}
\end{figure}

